Is News Recommendation a Sequential Recommendation Task?

News recommendation is often modeled as a sequential recommendation task, which assumes that there are rich short-term dependencies over historical clicked news. However, in news recommendation scenarios users usually have strong preferences on the temporal diversity of news information and may not tend to click similar news successively, which is very different from many sequential recommendation scenarios such as e-commerce recommendation. In this paper, we study whether news recommendation can be regarded as a standard sequential recommendation problem. Through extensive experiments on two real-world datasets, we find that modeling news recommendation as a sequential recommendation problem is suboptimal. To handle this challenge, we further propose a temporal diversity-aware news recommendation method that can promote candidate news that are diverse from recently clicked news, which can help predict future clicks more accurately. Experiments show that our approach can consistently improve various news recommendation methods.

==> data/related.tex <==
\section{Related Work}

\subsection{Transformer and Self-Attention}

The Transformer model is built upon multi-head self-attention, which can effectively models the contexts within a sequence by capturing the interactions between the inputs at each pair of positions~\cite{vaswani2017attention}.
An $h$-head self-attention mechanism can be formulated as follows:
\begin{equation}
\begin{aligned}
    &\rm{MultiHead}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) =\\ 
    &\rm{Concat}(\rm{head}_1, \rm{head}_2, ..., \rm{head}_h)\mathbf{W}^O,
\end{aligned}
\end{equation}
where $\mathbf{Q}$, $\mathbf{K}$, $\mathbf{V}\in \mathbb{R}^{N\times d}$ are the input query, key and value matrices, $N$ is the sequence length, $d$ is the hidden dimension in each attention head, and $\mathbf{W}^O\in \mathbb{R}^{hd\times d}$ is a linear transformation parameter matrix.
The representation learned by each attention head is formulated as follows:
\begin{equation}
\begin{aligned}
    \rm{head}_i&= \rm{Attention}(\mathbf{Q}\mathbf{W}^Q_i,\mathbf{K}\mathbf{W}^K_i,\mathbf{V}\mathbf{W}^V_i)\\ 
    &=\rm{softmax}(\frac{\mathbf{Q}\mathbf{W}^Q_i(\mathbf{K}\mathbf{W}^K_i)^T}{\sqrt{d}})\mathbf{V}\mathbf{W}^V_i,
\end{aligned}
\end{equation}
where $\mathbf{W}^Q_i$, $\mathbf{W}^K_i$, $\mathbf{W}^V_i\in \mathbb{R}^{d\times d}$ are learnable parameters.
From this formula, we can see that the computational complexity is quadratic to the sequence length $N$.
It has become a bottleneck for Transformers to handle long sequences.



\subsection{Efficient Transformer}

In recent years, there are many approaches to improving the efficiency of Transformer architecture~\cite{tay2020efficient}.
Some methods use sparse attention mechanisms to reduce the complexity of self-attention~\cite{child2019generating,beltagy2020longformer,zaheer2020big,zhang2021pooling}.
For example, Longformer~\cite{beltagy2020longformer} uses sliding window attention to attend local contexts and uses global attention on a few pre-selected input locations to capture global contexts.
BigBird~\cite{zaheer2020big} combines local attention, global attention at certain positions and random attention on several randomly selected token pairs.
However, these methods may need a relative larger  number of attended tokens to reduce the performance degradation on longer sequences, which usually lead to a limited speed-up ratio.

Another way is using hashing technique to accelerate self-attention computation.
For example, Reformer~\cite{Kitaev2020reformer} uses a multi-round hashing scheme to put similar representations into same buckets when computing self-attention, which can theoretically reduce the complexity to $O(N\log(N))$.
However, the computational complexity constant of Reformer is quite large, making it inefficient in processing common sequences with rather limited lengths.

There are also several methods that aim to reduce the computational cost by computing approximated  self-attention~\cite{choromanski2020masked,wang2020linformer,tay2021synthesizer}.
For instance, Linformer~\cite{wang2020linformer} projects the attention key and value into low-rank matrices to approximate the self-attention mechanism.
Linear Transformer~\cite{katharopoulos2020transformers} uses a kernel-based formulation of self-attention and the associative
property of matrix multiplication to approximate the dot-product attention.
However, these methods approximate self-attention in a context-agnostic manner, which may not be optimal for text modeling. 
In addition, they still bring heavy computational cost when the sequence length is very long.
Different from the aforementioned methods, \textit{Fastformer} uses additive attention to model global contexts and uses element-wise product to model the interaction between each input representation and global contexts, which can greatly reduce the computational cost and meanwhile effectively capture contextual information. 

